Saying Hello World with Epsilon - A Solution to the 2011 Instructive Case

Epsilon is an extensible platform of integrated and task-specific languages for model management. With solutions to the 2011 TTC Hello World case, this paper demonstrates some of the key features of the Epsilon Object Language (an extension and reworking of OCL), which is at the core of Epsilon. In addition, the paper introduces several of the task-specific languages provided by Epsilon including the Epsilon Generation Language (for model-to-text transformation), the Epsilon Validation Language (for model validation) and Epsilon Flock (for model migration).

==> eptcsdata.tex <==
\providecommand{\firstpage}{332}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.27}{10.4204/EPTCS.74.27}}
\pdfoutput=1

